Analogue Hawking radiation as a tunneling in a two-level $\mathcal{PT}$-symmetric system

In the light of a general scenario of a two-level non-Hermitian $\mathcal{PT}$-symmetric Hamiltonian we apply the tetrad-based method to analyze the possibility of analogue Hawking radiation. It is done by making use of the conventional null-geodesic approach wherein the associated Hawking radiation is described as a quantum tunneling process across a classically forbidden barrier which the event horizon imposes. An interesting aspect of our result is that our estimate for the tunneling probability is independent of the non-Hermitian parameter that defines the guiding Hamiltonian.

==> Structure.tex <==
% ---------------------- PACKAGES AND MORE ----------------------


% ========================================================
%           Various
% ========================================================

\usepackage[utf8]{inputenc}

\usepackage[top=3.5cm,bottom=3.5cm, left=4cm,right=4cm,   heightrounded,marginparwidth=1.5cm, marginparsep=1cm]{geometry} %for margins

\usepackage[shortlabels]{enumitem} % for lists

\usepackage[square,numbers,merge,comma,sort&compress]{natbib} % bibliography
\makeatletter
\def\NAT@spacechar{\,}  % define space inside [1,\,2]
\makeatother

\usepackage{amsmath,amssymb,amsfonts,amsthm,amsbsy,breqn}
\usepackage{mathtools} % for {rcases}

\usepackage{fnpct}% for multiple footnote at same point
\setfnpct{dont-mess-around} % no other kerning and punctuation switching

\usepackage{slashed,cancel,latexsym}
\usepackage{old-arrows,comment,relsize,setspace,moresize}
\usepackage{epsfig}
\usepackage{changepage,adjustbox}
\usepackage{mathrsfs,calligra,aurical,bold-extra} % fonts, \mathscr ...
\usepackage{calc,float,appendix}
\usepackage{bigints,xargs,extarrows}
\usepackage{empheq,soul} % for \hl{...}

\usepackage[svgnames]{xcolor}  % Load BEFORE tikz!
\definecolor{Blue}{rgb}{0.0, 0.0, 0.37}
\definecolor{Green}{rgb}{0.05, 0.45, 0.25}
\xdefinecolor{dogwoodrose}{rgb}{0.8, 0.1, 0.55}
\xdefinecolor{RRed}{rgb}{0.7, 0.1, 0.525}

\usepackage{tikz}
\usetikzlibrary{scopes,decorations.pathmorphing,patterns,calc,arrows,shapes.geometric,shapes.arrows,decorations.markings,plotmarks}
\usepackage{pgfplots}

\usepackage[blocks]{authblk}  % authors and affiliations
\renewcommand\Authfont{\normalfont\normalsize\bfseries%\scshape
}
\renewcommand\Authsep{, }
\renewcommand\Authand{, }
\renewcommand\Authands{, }
\renewcommand\Affilfont{\normalfont\footnotesize}
\setlength{\affilsep}{1em} % spacing between lines


% ======================================================
%                Images, graphics, tables
% ======================================================

\usepackage{graphicx} % Required for including images
\graphicspath{{Figures/}} % Set the default folder for images

\usepackage[labelsep=colon]{caption}  % captions
\captionsetup[figure]{format=hang,font={small,stretch=1.2},labelfont=small}
\captionsetup[table]{aboveskip=10pt,belowskip=15pt}

\usepackage[labelsep=colon,aboveskip=10pt,belowskip=10pt]{subcaption}
\captionsetup[sub]{format=hang,labelformat=simple,aboveskip=5pt,belowskip=15pt}
\DeclareCaptionSubType * [roman]{table}
\captionsetup[subtable]{format=hang,labelformat=simple,aboveskip=5pt,belowskip=0pt}

\usepackage{array,tabularx}

% ======================================================
%           Sections and TOC
% ======================================================

\usepackage{titlesec}
%\titleformat{command}[shape]{format}{label}{sep}{before-code}[after-code]
\titleformat{\section}{\normalfont\fontsize{12.5}{12}\bfseries}{\thesection}{0.5em}{}%{\phantomsection}
\titleformat{\subsection}{\normalfont\fontsize{10.5}{10}\bfseries}{\thesubsection}{0.5em}{}%{\phantomsection}
\titleformat{\subsubsection}{\normalfont\normalsize\bfseries}{\thesubsubsection}{0.5em}{}%{\phantomsection}

%\titlespacing*{<command>}{<left>}{<before-sep>}{<after-sep>}[right-sep]
\titlespacing*{\section}{0pt}%
                {4ex plus 1ex minus .5ex}{1.75ex plus .25ex minus .25ex}
\titlespacing*{\subsection}{0pt}%
                {3.5ex plus 1ex minus .5ex}{1.25ex plus .2ex minus .2ex}
\titlespacing*{\subsubsection}{0pt}%
                {2.5ex plus 0.75ex minus .2ex}{0.75ex plus .15ex minus .15ex}
\titlespacing*{\paragraph}{0pt}%
                {1.85ex plus 0.5ex minus .15ex}{1em}


\usepackage{titletoc}
\addtocontents{toc}{\addvspace{-0.75em}}  % reduce vert space before TOC
%\setcounter{secnumdepth}{0} % labeling depth.  Sections are lev. 1
\setcounter{tocdepth}{2}     % depth of table of cont. (sec, subsect ...)


\makeatletter
\patchcmd{\@maketitle}{\begin{center}}{\begin{adjustwidth}{-0.25in}{-0.25in}\begin{center}}{}{}
\patchcmd{\@maketitle}{\end{center}}{\end{center}\end{adjustwidth}}{}{}
\makeatother



%\renewcommand\refname{\normalsize{References}}


% ======================================================
%        Alphabets
% ======================================================

\newcommand\hmmax{1}
\newcommand\bmmax{1} % don't load too much alphabets in bm,bbm
\usepackage{bm}  % \mathbbm only has digits "1" and "2"
%\usepackage{bbm}
\usepackage{dsfont}  % double math characters (but only digit "1")

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\DeclareSymbolFontAlphabet{\Scr}{rsfs}
\DeclareMathAlphabet{\mathbold}{U}{BOONDOX-ds}{m}{n}
\SetMathAlphabet{\mathbold}{bold}{U}{BOONDOX-ds}{b}{n}
\DeclareMathAlphabet{\mathcalboondox}{U}{BOONDOX-calo}{m}{n}
\SetMathAlphabet{\mathcalboondox}{bold}{U}{BOONDOX-calo}{b}{n}
\DeclareMathAlphabet{\mathbcalboondox}{U}{BOONDOX-calo}{b}{n}


% Symbols From mathabx package
\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{ <5> <6> <7> <8> <9> <10> gen * matha
                    <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12}{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}
\DeclareMathSymbol{\varleftarrow}{3}{matha}{"D0}
\DeclareMathSymbol{\varrightarrow}{3}{matha}{"D1}
\DeclareMathSymbol{\simeq}{3}{matha}{"14}
\DeclareMathSymbol{\sim}{3}{matha}{"12}
\DeclareMathSymbol{\ll}{3}{matha}{"21}
\DeclareMathSymbol{\gtrsim}{3}{matha}{"C1}
\DeclareMathSymbol{\lesssim}{3}{matha}{"C0}


% ======================================================
%          Back references setup
% ======================================================

\newcommand\linkcol{RRed}
\newcommand\eqcol{black}


%% Load it HERE, after_other_packages !!!!!!!!!
\usepackage[breaklinks=true,backref=page]{hyperref}
\hypersetup{
    bookmarks=true,         % show bookmarks bar?
    bookmarksnumbered=true,
    %unicode=false,          % non-Latin characters in Acrobat’s bookmarks
    pdftoolbar=true,        % show Acrobat’s toolbar?
    pdfmenubar=true,        % show Acrobat’s menu?
    pdffitwindow=false,     % window fit to page when opened
%    pdfstartview={FitW},    % fits the width of the page to the window
%    pdftitle={Certificate},    % title
    pdfauthor={},     % author
    pdfsubject={},   % subject of the document
    pdfcreator={},   % creator of the document
    pdfproducer={},  % producer of the document
%    pdfkeywords={Certificates,} {TEQIP} {Participation}, % list of keywords
%    pdfnewwindow=true,      % links in new window
%
    pdfpagemode={UseNone},
    pdfstartview={FitH},
    colorlinks=true,
    plainpages,
%    a4paper,
    linktoc=page,
    citecolor=blue,
    filecolor=black,
    linkcolor=\linkcol,
    urlcolor=Grey,
}
\renewcommand*{\backref}[1]{}
\renewcommand*{\backrefalt}[4]{%
\ifcase #1 %
\relax
\or
~{\small [\textsc{p.~\fns{\!#2}}]}
\else
~{\small [\textsc{p.~\fns{\!#2}}]}%
\fi}
\renewcommand*{\backrefsep}{,\,}
\renewcommand*{\backreftwosep}{,\,}
\renewcommand*{\backreflastsep}{,\,}


\usepackage{footnotebackref}
\usepackage{hypernat} % Load it HERE, after NATBIB and HYPERREF
                      %  it is used for correct backreferences

\usepackage{cleveref} % Load it HERE, after HYPERREF
\newcommand{\crefrangeconjunction}{--}



% ======================================================
%            Layout
% ======================================================

\makeatletter
%\linespread{1.175}
\renewcommand{\baselinestretch}{1.125}\normalsize
\setlength\lineskip{1pt}
\setlength\parindent{1.2\parindent}
\setlength\normallineskip{1pt}
\setlength\parskip{0.75pt \@plus 0.75pt}
\setlength{\skip\footins}{22pt plus 5pt minus 5pt}
\setlength{\footnotesep}{8pt plus 2pt minus 1pt}
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
\widowpenalty 1000
\clubpenalty 1000
%
%\voffset -1in
%\topmargin   .05\paperheight
%\headheight  .02\paperheight
%\headsep     .03\paperheight
%\footskip    .07\paperheight
%
%\marginparsep 9pt
%\marginparpush 6pt
%
%\hoffset -1in
%\oddsidemargin .14\paperwidth
%\evensidemargin .14\paperwidth
%\marginparwidth .11\paperwidth
%
%\interdisplaylinepenalty=2500
%\relpenalty=9999
%\binoppenalty=9999
\interfootnotelinepenalty=10000
\makeatother


\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother


% ======================================================
%            Define commands
% ======================================================

\def\+{~+~}
\def\-{~-~}
\def\={\:=\:}
\newcommand\fns{\footnotesize}
\newcommand\nn{\nonumber}
\newcommand\Real{\textrm{Re}}
\newcommand\Img{\textrm{Im}}
\newcommand\Id{\mathds{1}}
\newcommand\Zero{\mathbold{0}}
\newcommandx\Hodge[1][1=4,usedefault]{{}^{\star_{#1}}}

\newcommand\ux{\vec{u}_x}
\newcommand\uy{\vec{u}_y}
\newcommand\uz{\vec{u}_z}

\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}




\newcommandx{\overbar}[1]{\mkern
1.5mu\overline{\mkern-2.0mu#1\mkern-2.0mu}\mkern 1.5mu}
\newcommandx{\overbarcal}[1]{\mkern                   6.0mu\overline{\mkern-5.5mu#1\mkern-1.0mu}\mkern 1.5mu}


% % \usepackage[utf8]{inputenc}
% % \usepackage[dvips]{color}
% % \usepackage[toc]{appendix}
% % \usepackage[hang,flushmargin]{footmisc} 
% \usepackage{titlesec,titletoc,ntheorem-hyper,authblk,abstract,latexsym,microtype,booktabs,amsmath,cleveref,fancyhdr,wrapfig,array,amsfonts, amssymb,geometry,appendix,cite}\geometry{margin=3cm}

% \renewcommand{\abstractname}{}
% \renewcommand{\absnamepos}{empty}
% % \renewcommand\Authands{ and }
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\C}{\mathbb{C}}

% % \newcommand{\be}{\begin{equation}}
% % \newcommand{\ee}{\end{equation}}
% % \newcommand{\bea}{\begin{eqnarray}}
% % \newcommand{\eea}{\end{eqnarray}}
% % \newcommand\blfootnote[1]{%
% %   \begingroup
% %   \renewcommand\thefootnote{}\footnote{#1}%
% %   \addtocounter{footnote}{-1}%
% %   \endgroup
% % }

% \usepackage{graphicx,lipsum}
% \usepackage{caption}
% \usepackage{subfigure}
% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{amssymb}
% \usepackage{stackengine}
% \usepackage{mathtools}
% % \numberwithin{equation}{section}
% % \usepackage{titlesec}
% \usepackage{sectsty}
% \sectionfont{\centering}
% \newtheorem{case}{Case:}
% \newtheorem{subcase}{Case}
% \numberwithin{subcase}{case}
% \usepackage{framed}
% \allowdisplaybreaks
% % \bibliographystyle{plain}
% \usepackage[nottoc]{tocbibind}
% \usepackage[free-standing-units]{siunitx}
% \usepackage{helvet}
% \usepackage{url}
% \usepackage{titletoc}
% \usepackage{blindtext}
% \usepackage[gen]{eurosym}
% \newcommand{\ackname}{Acknowledgements}
% \DeclareMathOperator{\E}{\mathbb{E}}

